Deep Learning-Aided Perturbation Model-Based Fiber Nonlinearity Compensation

Fiber nonlinearity effects cap achievable rates and ranges in long-haul optical fiber communication links. Conventional nonlinearity compensation methods, such as perturbation theory-based nonlinearity compensation (PB-NLC), attempt to compensate for the nonlinearity by approximating analytical solutions to the signal propagation over optical fibers. However, their practical usability is limited by model mismatch and the immense computational complexity associated with the analytical computation of perturbation triplets and the nonlinearity distortion field. Recently, machine learning techniques have been used to optimise parameters of PB-based approaches, which traditionally have been determined analytically from physical models. It has been claimed in the literature that the learned PB-NLC approaches have improved performance and/or reduced computational complexity over their non-learned counterparts. In this paper, we first revisit the acclaimed benefits of the learned PB-NLC approaches by carefully carrying out a comprehensive performance-complexity analysis utilizing state-of-the-art complexity reduction methods. Interestingly, our results show that least squares-based PB-NLC with clustering quantization has the best performance-complexity trade-off among the learned PB-NLC approaches. Second, we advance the state-of-the-art of learned PB-NLC by proposing and designing a fully learned structure. We apply a bi-directional recurrent neural network for learning perturbation triplets that are alike those obtained from the analytical computation and are used as input features for the neural network to estimate the nonlinearity distortion field. Finally, we demonstrate through numerical simulations that our proposed fully learned approach achieves an improved performance-complexity trade-off compared to the existing learned and non-learned PB-NLC techniques.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> References.tex <==

\bibitem{ASharma2021}
A. Sharma, A. Jain, P. Gupta, and V. Chowdary, “Machine learning applications for precision agriculture: a comprehensive review,” \textit{IEEE Access}, vol. 9, pp. 4843-4873, Jan. 2021. DOI: 10.1109/ACCESS.2020.3048415.

\bibitem{DBertsimas2021}
D. Bertsimas, L. Mingardi, and B. Stellato, “Machine learning for real-time heart disease prediction
,” \textit{IEEE J. Biomed. Health Inform.}, vol. 25, no. 9, pp.  3627-3637, Sep. 2021.

\bibitem{DChen2021} 
D. Chen, N. Chen, X. Zhang, H. Ma, and Z. Chen, “Next-generation soil moisture sensor web: high-density in situ observation over NB-IoT,” \textit{IEEE Internet Things J.}, vol. 8, no. 17, pp. 13367-13383, Sep. 2021. 

\bibitem{SHu2021}
S. Hu, X. Chen, W. Ni, E. Hossain, and X. Wang, “Distributed machine learning for wireless communication networks: techniques, architectures, and applications,” \emph{IEEE Commun. Surv. Tutorials}, vol. 23, no. 3, pp. 1458-14933, Jun. 2021.

\bibitem{DRafique2016}
D. Rafique, “Fiber nonlinearity compensation: commercial applications and complexity analysis,” \emph{IEEE/OSA J. Lightw. Technol.}, vol. 34, no. 2, pp. 544-553, Jan. 2016.

\bibitem{PJWinzer2017}
P. J. Winzer and D. T. Neilson, “From scaling disparities to integrated parallelism: a decathlon for a decade,” \emph{IEEE/OSA J. Lightw. Technol.}, vol. 35, no. 5, pp. 1099-1115, Mar. 2017.

\bibitem{RJEssiambr2010}
R. J. Essiambre, G. Kramer, P. J. Winzer, G. J. Foschini, and B. Goebel, “Capacity limits of optical fiber networks,” \emph{IEEE/OSA J. Lightw. Technol.}, vol. 28, no. 4, pp. 662-701, Feb. 2010.

\bibitem{Amari2017}
A. Amari, O. A. Dobre, R. Venkatesan, O. S. Sunish Kumar, P. Ciblat, and Y. Jaouën, “A survey on fiber nonlinearity compensation for 400 Gbps and beyond optical communication systems,” \emph{IEEE Commun. Surv. Tutorials}, vol. 19, no. 4, pp. 3097-3113, 4th Quart. 2017.

\bibitem{SKOSoman2021}
S. K. O. Soman, A. Amari, O. A. Dobre, and R. Venkatesan, “Second-order perturbation theory-based digital predistortion for fiber nonlinearity compensation,” \emph{IEEE/OSA J. Lightw. Technol.}, vol. 39, no. 17, pp. 5474-5485, Sep. 2021.

\bibitem{SunishKumar2017}
O. S. Sunish Kumar, O. A. Dobre, R. Venkatesan, S. K. Wilson, O. Omomukuyo, A. Amari, and D. Chang, “A spectrally-efficient linear polarization coding scheme for fiber nonlinearity compensation in CO-OFDM systems,” in \emph{Proc. SPIE Opt.}, vol. 10130, pp. 1-10, Jan. 2017.

\bibitem{Sunish2018}
A. Amari, L. Lampe, O. S. Sunish Kumar, Y. C. Gültekin, and A. Alvarado, “Comparison of short blocklength sphere shaping and nonlinearity compensation in WDM systems,” \emph{IEEE Photon. Technol. Lett.}, vol. 32, no. 22, pp. 1435-1438, Nov. 2020.

% \bibitem{Sunish2018}
% O. S. Sunish Kumar, A. Amari, O. A. Dobre, and R. Venkatesan, “PDL impact on linearly coded digital phase conjugation techniques in CO-OFDM systems,” \emph{IEEE Photon. Technol. Lett.}, vol. 30, no. 9, pp. 769-772, May 2018. 

\bibitem{Vassilieva2019}
O. Vassilieva, I. Kim, and T. Ikeuchi, “Enabling technologies for fiber nonlinearity mitigation in high capacity transmission systems,” \emph{IEEE/OSA J. Lightw. Technol.}, vol. 37, no. 1, pp. 50-60, Jan. 2019.

\bibitem{Sunish2017}
O. S. Sunish Kumar, A. Amari, O. A. Dobre, R. Venkatesan, and S. K. Wilson, “A joint technique for nonlinearity compensation in CO-OFDM superchannel systems,” in \emph{Proc. ACPC}, Nov. 2017, paper Su4B.4.

\bibitem{OSSunishKumar2020}
O. S. Sunish Kumar, A. Amari, O. A. Dobre, and R. Venkatesan, “Intra-channel nonlinearity compensation based on second-order perturbation theory,” arXiv:2005.01191v1 [cs.IT], May 2020. 

\bibitem{SunishThesis}
O. S. Sunish Kumar, “Digital Signal Processing Techniques for Fiber Nonlinearity Compensation in Coherent Optical Communication Systems,” Ph.D thesis, Memorial University of Newfoundland, Canada, 2020.

\bibitem{TTNguyen}
T. T. Nguyen, P. Harper, O. S. Sunish Kumar, and A. Ellis, “Nonlinear tolerance enhancement based on perturbation theory for optical phase conjugation systems,” in \emph{Proc. OFC}, Mar. 2020, paper Th2A.52. 

\bibitem{OSSunishKumar2019}
O. S. Sunish Kumar, A. Amari, O. A. Dobre, and R. Venkatesan, “Enhanced regular perturbation-based
nonlinearity compensation technique for optical transmission systems,” \emph{IEEE Photon. J.}, vol. 11, no. 4, pp. 1-13, Aug. 2019.

\bibitem{Ip2008}
E. Ip and J. M. Kahn, “Compensation of dispersion and nonlinear impairments using digital backpropagation,” \emph{IEEE/OSA J. Lightw. Technol.}, vol. 26, no. 20, pp. 3416-3425, Oct. 2008.

\bibitem{JCCartledge2017}
J. C. Cartledge, F. P. Guiomar, F. R. Kschischang, G. Liga, and M. P. Yankov, “Digital signal processing for fiber nonlinearities,” \emph{Opt. Express}, vol. 25, no. 3, pp. 1916-1936, Feb. 2017.

\bibitem{Vannucci2002}
A. Vannucci, P. Serena, and A. Bononi, “The RP method: a new tool for the iterative solution of the nonlinear Schrödinger equation,” \emph{IEEE/OSA J. Lightw. Technol.}, vol. 20, no. 7, pp. 1102-1112, Jul. 2002.

\bibitem{V. Oliari2020}
V. Oliari, E. Agrell, and A. Alvarado, “Regular perturbation on the group-velocity dispersion parameter for nonlinear fibre-optical communications,” \textit{Nat. Commun.}, 11, 933 (2020), https://doi.org/10.1038/s41467-020-14503-w.

\bibitem{ARedyuk2020}
A. Redyuk, E. Averyanov, O. Sidelnikov, M. Fedoruk, and S. Turitsyn, “Compensation of nonlinear impairments using inverse perturbation theory with reduced complexity,” \emph{IEEE/OSA J. Lightw. Technol.}, vol. 38, no. 6, pp. 1250-1257, Mar. 2020. 

\bibitem{YGao2014}
Y. Gao, J. C. Cartledge, A. S. Karar, S. S. H. Yam, M. O’Sullivan, C. Laperle, A. Borowiec, and K. Roberts, “Reducing the complexity of perturbation based nonlinearity pre-compensation using symmetric EDC and pulse shaping,” \emph{Opt. Exp.}, vol. 22, no. 2, pp. 1209-1219, Jan. 2014. 

\bibitem{LDou2012}
L. Dou, Z. Tao, W. Yan, L. Li, T. Hoshida, and J. C. Rasmussen, “Pre-distortion method for intra-channel nonlinearity compensation with phase-rotated perturbation term,” in \emph{Proc. OFC}, Mar. 2012, paper OTh3C.2.

\bibitem{AMecozzi2000}
A. Mecozzi, C. B. Clausen, and M. Shtaif, “Analysis of intrachannel nonlinear effects in highly dispersed optical pulse transmission,” \emph{IEEE Photon. Technol. Lett.}, vol. 12, no. 4, pp. 392-394, Apr. 2000.

\bibitem{Tao2011}
Z. Tao, L. Dou, W. Yan, L. Li, T. Hoshida, and J. C. Rasmussen, “Multiplier-free intrachannel nonlinearity compensating algorithm operating at symbol rate,” \emph{IEEE/OSA J. Lightw. Technol.}, vol. 29, no. 17, pp. 2570-2576, Sep. 2011.

\bibitem{YZhao2013ECOC}
Y. Zhao, L. Dou, Z. Tao, M. Yan, S. Oda,
T. Tanimura, T. Hoshida, and J. C. Rasmussen, \textquotedblleft Improved analytical model for intra-channel nonlinear distortion by relaxing the lossless assumption,\textquotedblright{} in \textit{Proc. ECOC}, London, UK, Sep. 2013, paper P.4.16.

\bibitem{Tao2015JLT}
Z. Tao, L. Dou, W. Yan, L. Li, T. Hoshida, and J. C. Rasmussen, “Analytical intra-channel nonlinear models
to predict the nonlinear noise waveform,” \emph{IEEE/OSA J. Lightw. Technol.}, vol. 33, no. 10, pp. 2111-2119, May 2015.

\bibitem{FFrey2018ECOC}
F. Frey, R. Emmerich, C. Schubert, J. K. Fischer, and R. F. H. Fischer, \textquotedblleft Improved Perturbation-based Fiber Nonlinearity Compensation,\textquotedblright{} in \textit{Proc. ECOC}, Rome, Italy, Nov. 2018, doi: 10.1109/ECOC.2018.8535303.

\bibitem{Liang2014}
X. Liang and S. Kumar, “Multi-stage perturbation theory for compensating intra-channel nonlinear impairments in fiber-optic links,” \emph{Opt. Express}, vol. 22, no. 24, pp. 29733-29745, Nov. 2014.

\bibitem{RMButler2020}
R. M. B\"{u}tler, C. Häger, H. D. Pfister, G. Liga, A. Alvarado, “Model-based machine learning for joint digital backpropagation and PMD compensation,” \emph{IEEE/OSA J. Lightw. Technol.}, vol. 39, no. 4, pp. 949-959, Feb. 2021.

\bibitem{SZhang2019}
S. Zhang, F. Yaman, K. Nakamura, T. Inoue, V. Kamalov, L. Jovanovski, V. Vusirikala, E. Mateo, Y. Inada, and T. Wang, “Field and lab experimental demonstration of nonlinear impairment compensation using neural networks,” in in \emph{Nat. Commun.}, 2019, https://doi.org/10.1038/s41467-019-10911-9.

\bibitem{YGao2019}
Y. Gao, Z. A. El-Sahn, A. Awadalla, D. Yao, H. Sun, P. Mertz, and K. T. Wu, “Reduced complexity nonlinearity compensation via principal component analysis and deep neural networks,” in in \emph{Proc. OFC}, Mar. 2019, paper Th2A.49. 

\bibitem{CHager2018}
C. H\"{a}ger and H. D. Pfister, “Nonlinear interference mitigation via deep neural networks,” in \emph{Proc. OFC}, Mar. 2018, paper W3A.4. 

\bibitem{Fougstedt2018}
C. Fougstedt, C. H\"{a}ger, L. Svensson, H. D. Pfister, and P. Larsson-Edefors, “ASIC implementation of time-domain digital backpropagation with deep-learned chromatic dispersion filters,”
in \emph{Proc. ECOC}, 2018, pp. 1–3.

\bibitem{CHager2020}
C. H\"{a}ger, H. D. Pfister, R. M. Butler,
G. Liga, and A. Alvarado, “Model-based machine learning for joint digital backpropagation and PMD compensation,” in \emph{Proc. OFC}, Mar. 2020, paper W3D.3. 

\bibitem{OSSKumarSPPCom2021}
O. S. S. Kumar, L. Lampe, S. Luo, M. Jana, J. Mitra, and C. Li, “Deep neural network assisted second-order
perturbation-based nonlinearity compensation,” in \emph{Proc. SPPCom.}, Jul. 2021, paper SpF2E.2.

\bibitem{YZhao2020Access}
Y. Zhao, X. Chen, T. Yang, L. Wang, D. Wang, Z. Zhang, and S. Shi “Low-complexity fiber nonlinearity impairments compensation enabled by simple recurrent neural network with time memory,” \textit{IEEE Access}, vol. 8, pp. 160995-1610043, Sep. 2020. DOI: 10.1109/ACCESS.2020.3021146.

\bibitem{Lietal}
C. Li, Y. Wang, J. Wang, H. Yao, X. Liu, R. Gao, L. Yang, H. Xu, Q. Zhang, P. Ma, and X. Xin “Convolutional Neural Network-Aided {DP-64 QAM} Coherent Optical Communication Systems,” \textit{Journal of Lightwave Technology}, vol. 40, no. 9, pp. 2880-2889, 2022, DOI: 10.1109/JLT.2022.3146839.

\bibitem{Malekiha2016}
M. Malekiha and D. V. Plant, “Adaptive optimization of quantized perturbation coefficients for fiber nonlinearity compensation,” \emph{IEEE Photon. J.}, vol. 8, no. 3, pp. 17, Jun. 2016.

\bibitem{LTH}
A. Renda, J. Frankle and M. Carbin, "Comparing Rewinding and Fine-tuning in Neural Network Pruning," \textit{International Conference on Learning Representations}, 2020

\bibitem{Bengio}
Y. Bengio and P. Simard and P. Frasconi, "Learning long-term dependencies with gradient descent is difficult," \textit{IEEE Transactions on Neural Networks}, vol. 5, no. 2, pp. 157-166, 1994, DOI: 10.1109/72.279181.

\bibitem{Gers}
F. Gers, “Long Short-Term Memory in Recurrent Neural Networks,” Ph.D thesis, {\'E}cole Polytechnique F{\'e}d{\'e}ral de Laussane, Switzerland, 2001.

\bibitem{ZTao2013}
Z. Tao, L. Dou, W. Yan, Y. Fan, L. Li, S. Oda,
Y. Akiyama, H. Nakashima, T. Hoshida, and J. C. Rasmussen, “Complexity-reduced digital nonlinear compensation for coherent optical systems,” in \emph{Proc. SPIE Opt.}, San Francisco, CA, USA, pp. 115-125, Jan. 2013.

\bibitem{JOSunish2021}
O. S. Sunish Kumar “A tutorial on fiber Kerr nonlinearity effect and its compensation in optical communication systems,” \textit{Journal of Optics}, vol. 23, no. 12, 2021.

\bibitem{OurECOC}
S. Luo, O. S. Sunish Kumar, L. Lampe, M. Jeebak, and C. Li,
\textquotedblleft Learning for Perturbation-Based Fiber Nonlinearity Compensation,\textquotedblright{} in \textit{Proc. ECOC}, 2022.

\bibitem{Diedolo}
F. Diedolo, G. B\"{o}cherer, M. Sch\"{a}dler, and S. Calabró, “Nonlinear Equalization for Optical Communications Based on Entropy-Regularized Mean Square Error,” arXiv:2206.01004 [cs.IT], June 2022.

\bibitem{Ming2022}
H. Ming, X. Chen, X. Fang, L. Zhang, C. Li and F. Zhang, "Ultralow Complexity Long Short-Term Memory Network for Fiber Nonlinearity Mitigation in Coherent Optical Communication Systems," \emph{IEEE/OSA J. Lightw. Technol.}, vol. 40, no. 8, pp. 2427-2434, April 2022, doi: 10.1109/JLT.2022.3141404.

==> References_Sample.tex <==
\bibitem{MChen2019}
M. Chen, W. Saad, C. Yin, and M. Debbah, “Data correlation-aware resource management in wireless virtual reality (VR): an echo state transfer learning approach,” \textit{IEEE Trans. Commun.}, vol. 67, no. 6, pp. 4267-4280, Jun. 2019.

\bibitem{JZhang2019} 
J. Zhang, S. Rajendran, Z. Sun, R. Woods, and L. Hanzo, “Physical layer security for the internet of things: authentication and key generation,” \textit{IEEE Wirel. Commun.}, vol. 26, no. 5, pp. 92-98, Oct. 2019.

\bibitem{FRestuccia2018} 
F. Restuccia, S. D’Oro, and T. Melodia, “Securing the internet of things in the age of machine learning and software-defined networking,” \textit{IEEE Internet Things J.}, vol. 5, no. 6, pp. 4829-4842, Dec. 2018.

\bibitem{Infinera2020}
Drivers for Coherent Transport Evolution, “The ultimate guide to higher baud rates,” \textit{Infinera White Paper}, 2020.

\bibitem{Amari2017}
A. Amari, O. A. Dobre, R. Venkatesan, O. S. Sunish Kumar, P. Ciblat, and Y. Jaouën, “A survey on fiber nonlinearity compensation for 400 Gbps and beyond optical communication systems,” \emph{IEEE Commun. Surv. Tutorials}, vol. 19, no. 4, pp. 3097-3113, 4th Quart. 2017.

\bibitem{SunishKumar2017}
O. S. Sunish Kumar, O. A. Dobre, R. Venkatesan, S. K. Wilson, O. Omomukuyo, A. Amari, and D. Chang, “A spectrally-efficient linear polarization coding scheme for fiber nonlinearity compensation in CO-OFDM systems,” in \emph{Proc. SPIE Opt.}, vol. 10130, pp. 1-10, Jan. 2017.

\bibitem{Sunish2018}
A. Amari, L. Lampe, O. S. Sunish Kumar, Y. C. Gültekin, and A. Alvarado, “Comparison of short blocklength sphere shaping and nonlinearity compensation in WDM systems,” \emph{IEEE Photon. Technol. Lett.}, vol. 32, no. 22, pp. 1435-1438, Nov. 2020.

% \bibitem{Sunish2018}
% O. S. Sunish Kumar, A. Amari, O. A. Dobre, and R. Venkatesan, “PDL impact on linearly coded digital phase conjugation techniques in CO-OFDM systems,” \emph{IEEE Photon. Technol. Lett.}, vol. 30, no. 9, pp. 769-772, May 2018. 

\bibitem{OSSKumarSPPCom2021}
O. S. S. Kumar, L. Lampe, S. Luo, M. Jana, J. Mitra, and C. Li, “Deep neural network assisted second-order
perturbation-based nonlinearity compensation,” in \emph{Proc. SPPCom.}, Jul. 2021, paper SpF2E.2.

\bibitem{Vassilieva2019}
O. Vassilieva, I. Kim, and T. Ikeuchi, “Enabling technologies for fiber nonlinearity mitigation in high capacity transmission systems,” \emph{IEEE/OSA J. Lightw. Technol.}, vol. 37, no. 1, pp. 50-60, Jan. 2019.

\bibitem{Liang2014}
X. Liang and S. Kumar, “Multi-stage perturbation theory for compensating intra-channel nonlinear impairments in fiber-optic links,” \emph{Opt. Express}, vol. 22, no. 24, pp. 29733-29745, Nov. 2014.

\bibitem{JCCartledge2017}
J. C. Cartledge, F. P. Guiomar, F. R. Kschischang, G. Liga, and M. P. Yankov, “Digital signal processing for fiber nonlinearities,” \emph{Opt. Express}, vol. 25, no. 3, pp. 1916-1936, Feb. 2017.

\bibitem{Ip2008}
E. Ip and J. M. Kahn, “Compensation of dispersion and nonlinear impairments using digital backpropagation,” \emph{IEEE/OSA J. Lightw. Technol.}, vol. 26, no. 20, pp. 3416-3425, Oct. 2008.

\bibitem{Sunish2017}
O. S. Sunish Kumar, A. Amari, O. A. Dobre, R. Venkatesan, and S. K. Wilson, “A joint technique for nonlinearity compensation in CO-OFDM superchannel systems,” in \emph{Proc. ACPC}, Nov. 2017, paper Su4B.4.

\bibitem{Peddanarappagari1997}
K. V. Peddanarappagari and M. Brandt-Pearce, “Volterra series transfer function of single-mode fibers,” \emph{IEEE/OSA J. Lightw. Technol.}, vol. 215, no. 12, pp. 2232-2241, Dec. 1997.

\bibitem{Guiomar2011}
F. P. Guiomar, J. D. Reis, A. L. Teixeira, and A. N.  Pinto, “Digital postcompensation using Volterra series transfer function,” \emph{IEEE Photon. Technol. Lett.}, vol. 23, no. 19, pp. 1412-1414, Oct. 2011.

\bibitem{AAmariICTON2017}
A. Amari,  O. A. Dobre, and R. Venkatesan, “Fifth-order Volterra series based nonlinear equalizer for long-haul high data rate optical fiber communications,” in \emph{Proc. IEEE ICTON}, Jan. 2017, paper We.A1.2.

\bibitem{VgenopoulouACPC2014}
V. Vgenopoulou, A. Amari, M. Song, E. Pincemin, I. Roudas, and Y. Jaouën, “Volterra-based nonlinear compensation in 400 Gb/s WDM multiband coherent optical OFDM systems,” in \emph{Proc. ACPC}, Nov. 2014, paper AF1E. 4.

\bibitem{ABakhshali2016}
A. Bakhshali, W. Y. Chan, J. C. Cartledge, M. O'Sullivan, C. Laperle, A. Borowiec, and K. Roberts, “Frequency-domain Volterra-based equalization structures for efficient mitigation of intrachannel Kerr nonlinearities,” \emph{IEEE/OSA J. Lightw. Technol.}, vol. 34, no. 8, pp. 1770-1777, Apr. 2016.

\bibitem{Diamantopoulos2019}
N. P. Diamantopoulos, H. Nishi, W. Kobayashi, K. Takeda, T. Kakitsuka, and S. Matsuo, “On the complexity reduction of the second-order Volterra nonlinear equalizer for IM/DD systems,” \emph{IEEE/OSA J. Lightw. Technol.}, vol. 37, no. 4, pp. 1214-1224, Feb. 2019.

\bibitem{Vannucci2002}
A. Vannucci, P. Serena, and A. Bononi, “The RP method: a new tool for the iterative solution of the nonlinear Schrödinger equation,” \emph{IEEE/OSA J. Lightw. Technol.}, vol. 20, no. 7, pp. 1102-1112, Jul. 2002.

\bibitem{V. Oliari2020}
V. Oliari, E. Agrell, and A. Alvarado, “Regular perturbation on the group-velocity dispersion parameter for nonlinear fibre-optical communications,” \textit{Nat. Commun.}, 11, 933 (2020), https://doi.org/10.1038/s41467-020-14503-w.

\bibitem{ARedyuk2020}
A. Redyuk, E. Averyanov, O. Sidelnikov, M. Fedoruk, and S. Turitsyn, “Compensation of nonlinear impairments using inverse perturbation theory with reduced complexity,” \emph{IEEE/OSA J. Lightw. Technol.}, vol. 38, no. 6, pp. 1250-1257, Mar. 2020. 

\bibitem{OSSunishKumar2020}
O. S. Sunish Kumar, A. Amari, O. A. Dobre, and R. Venkatesan, “Intra-channel nonlinearity compensation based on second-order perturbation theory,” arXiv:2005.01191v1 [cs.IT], May 2020. 

\bibitem{YGao2014}
Y. Gao, J. C. Cartledge, A. S. Karar, S. S. H. Yam, M. O’Sullivan, C. Laperle, A. Borowiec, and K. Roberts, “Reducing the complexity of perturbation based nonlinearity pre-compensation using symmetric EDC and pulse shaping,” \emph{Opt. Exp.}, vol. 22, no. 2, pp. 1209-1219, Jan. 2014. 

\bibitem{LDou2012}
L. Dou, Z. Tao, W. Yan, L. Li, T. Hoshida, and J. C. Rasmussen, “Pre-distortion method for intra-channel nonlinearity compensation with phase-rotated perturbation term,” in \emph{Proc. OFC}, Mar. 2012, paper OTh3C.2.

\bibitem{AMecozzi2000}
A. Mecozzi, C. B. Clausen, and M. Shtaif, “Analysis of intrachannel nonlinear effects in highly dispersed optical pulse transmission,” \emph{IEEE Photon. Technol. Lett.}, vol. 12, no. 4, pp. 392-394, Apr. 2000.

\bibitem{SunishThesis}
O. S. Sunish Kumar, “Digital Signal Processing Techniques for Fiber Nonlinearity Compensation in Coherent Optical Communication Systems,” Ph.D thesis, Memorial University of Newfoundland, Canada, 2020.

\bibitem{YGao2014}
Y. Gao, A. S. Karar, J. C. Cartledge, S. S. H. Yam, M. O’Sullivan, C. Laperle, A. Borowiec, and K. Roberts, “Joint pre-compensation and selective post-compensation for fiber nonlinearities,” \emph{IEEE Photon. Technol. Lett.}, vol. 26, no. 17, pp. 1746-1749, Jun. 2014.

\bibitem{T.Oyama2014}
T. Oyama, H. Nakashima, S. Oda, T. Yamauchi, Z. Tao, T. Hoshida, and J. C. Rasmussen, “Robust and efficient receiver side compensation method for intrachannel nonlinear effects,” in \emph{Proc. OFC}, Mar. 2014, paper Tu3A.3.

\bibitem{TTNguyen}
T. T. Nguyen, P. Harper, O. S. Sunish Kumar, and A. Ellis, “Nonlinear tolerance enhancement based on perturbation theory for optical phase conjugation systems,” in \emph{Proc. OFC}, Mar. 2020, paper Th2A.52.  

\bibitem{OSSunish Kumar2019}
O. S. Sunish Kumar, A. Amari, O. A. Dobre, and R. Venkatesan, “Enhanced regular perturbation-based
nonlinearity compensation technique for optical transmission systems,” \emph{IEEE Photon. J.}, vol. 11, no. 4, pp. 1-13, Aug. 2019.

\bibitem{Tao2011}
Z. Tao, L. Dou, W. Yan, L. Li, T. Hoshida, and J. C. Rasmussen, “Multiplier-free intrachannel nonlinearity compensating algorithm operating at symbol rate,” \emph{IEEE/OSA J. Lightw. Technol.}, vol. 29, no. 17, pp. 2570-2576, Sep. 2011.

\bibitem{DarFeder2016}
R. Dar, M. Feder, A. Mecozzi, and M. Shtaif, “Pulse Collision picture of inter-channel nonlinear
interference in fiber-optic communications,” \emph{IEEE/OSA J. Lightw. Technol.}, vol. 34, no. 2, pp. 593-607, Jan. 2016.

\bibitem{Vassilieva2018}
O. Vassilieva, “Enabling technologies for fiber nonlinearity mitigation in high capacity transmission systems,” in \emph{OFC}, Mar. 2018, tutorial Tu3G.1.

\bibitem{DarFeder2015}
R. Dar, M. Feder, A. Mecozzi, and M. Shtaif, “Inter-channel nonlinear interference noise in WDM
systems: modeling and mitigation,” \emph{IEEE/OSA J. Lightw. Technol.}, vol. 33, no. 5, pp. 1044-1053, Mar. 2015.

\bibitem{GhazisaeidiEssiambre2014}
A. Ghazisaeidi and R. J. Essiambre, \textquotedblleft Calculation of coefficients of perturbative nonlinear
pre-compensation for Nyquist pulses,\textquotedblright{} in \textit{Proc. ECOC}, Cannes, France, Sep. 2014, paper We.1.3.3.

\bibitem{OyamaNakashima2013}
T. Oyama, H. Nakashima, T. Hoshida, Z. Tao, C. Ohshima, and J. C. Rasmussen, \textquotedblleft Efficient transmitter-side nonlinear equalizer for 16QAM,\textquotedblright{} in \textit{Proc. ECOC}, London, UK, Sep. 2013, paper We.3.C.1.

\bibitem{ZTao2013}
Z. Tao, L. Dou, W. Yan, Y. Fan, L. Li, S. Oda,
Y. Akiyama, H. Nakashima, T. Hoshida, and J. C. Rasmussen, “Complexity-reduced digital nonlinear compensation for coherent optical systems,” in \emph{Proc. SPIE Opt.}, San Francisco, CA, USA, pp. 115-125, Jan. 2013.

\bibitem{NVIrukulapati2014}
N. V. Irukulapati, H. Wymeersch, P. Johannisson, and E. Agrell, “Stochastic digital backpropagation,” \textit{IEEE Trans. Commun.}, vol. 62, no. 11, pp. 3956-3968, Nov. 2014.

\bibitem{S. T. Le2015PCSC}
S. T. Le, M. E. McCarthy, N. M. Suibhne, M. A. Z. Al-Khateeb, E. Giacoumidis, N. Doran, A. D. Ellis, and S. K. Turitsyn, \textquotedblleft Demonstration of phase-conjugated subcarrier coding for fiber nonlinearity compensation in CO-OFDM transmission,\textquotedblright{} \textit{IEEE/OSA J. Lightw. Technol.}, vol. 33, no. 11, pp. 2206-2212, Jun. 2015.

\bibitem{LBomin2014}
L. Bomin, “Forward Error Correcting Codes for 100 Gbit/s Optical Communication Systems,” Ph.D thesis, Technical University of Denmark, Denmark, 2014.

\bibitem{Bengio}
Y. Bengio and P. Simard and P. Frasconi, "Learning long-term dependencies with gradient descent is difficult," \textit{IEEE Transactions on Neural Networks}, vol. 5, no. 2, pp. 157-166, 1994, DOI: 10.1109/72.279181.

\bibitem{Gers}
F. Gers, “Long Short-Term Memory in Recurrent Neural Networks,” Ph.D thesis, {\'E}cole Polytechnique F{\'e}d{\'e}ral de Laussane, Switzerland, 2001.

\bibitem{JOSunish2021}
O. S. Sunish Kumar “A tutorial on fiber Kerr nonlinearity effect and its compensation in optical communication systems,” \textit{Journal of Optics}, vol. 23, no. 12, 2021.

\bibitem{OurECOC}
S. Luo, O. S. Sunish Kumar, L. Lampe, M. Jeebak, and C. Li,
\textquotedblleft Learning for Perturbation-Based Fiber Nonlinearity Compensation,\textquotedblright{} in \textit{Proc. ECOC}, 2022.

\bibitem{Diedolo}
F. Diedolo, G. B\"{o}cherer, M. Sch\"{a}dler, and S. Calabró, “Nonlinear Equalization for Optical Communications Based on Entropy-Regularized Mean Square Error,” arXiv:2206.01004 [cs.IT], June 2022. 

\bibitem{Ming2022}
H. Ming, X. Chen, X. Fang, L. Zhang, C. Li and F. Zhang, "Ultralow Complexity Long Short-Term Memory Network for Fiber Nonlinearity Mitigation in Coherent Optical Communication Systems," \emph{IEEE/OSA J. Lightw. Technol.}, vol. 40, no. 8, pp. 2427-2434, April 2022, doi: 10.1109/JLT.2022.3141404.


==> maplestd2e.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% <PRE>
\def\MapleNameDef $#1: #2.#3${\expandafter\gdef\csname Maple@#1\endcsname{#2}}
\def\MapleInfoDef $#1: #2 #3${\expandafter\gdef\csname Maple@#1\endcsname{#2}}
\MapleNameDef $RCSfile: maple2e.sty,v $
\MapleInfoDef $Revision: 1.16 $
\MapleInfoDef $Date: 2005/03/17 15:58:14 $
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\typeout{Package: \Maple@RCSfile\space \Maple@Date\space v\Maple@Revision}
\ProvidesPackage{maplestd2e}[\Maple@Date\space\Maple@RCSfile
Maple Latex Style Package -- \Maple@Date\space\Maple@RCSfile]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Copyright (c) 1994--2005 by Waterloo Maple Inc., all rights reserved.
%
% Permission is granted to use this package without charge. It may
% be redistributed providing that it is distributed as is
% and without charge.  You may modify these macros for your own use,
% and redistribute them, subject to the following conditions.
%
% 1. The package name used for any modified version of this file is 
%    different from maple2e and the file name used is different from
%    maple2e.sty
%
% 2. You acknowledge this copyright notice and this file as the source.
%
% 3. The new file is redistributed under the same terms and conditions 
%    as indicated here, including a version of this notice modified to
%    refer to the new file and/or package name.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%
% Package:  maple2e 
%
% This package defines the latex macros used by "Export to LaTeX" 
% It makes use of several sub-packages.
% 
% mapleenv - Maple Environments used to mark mapleinput, mapleoutput,
% mapletab - Maple Macros to display tables (spreadsheets)
% mapleplots - Maple macros to display plots.
%
% See the comments in maplenv.sty for a more detailed discussion of
% the special environments such as
%
%	\begin{mapleinput} ... \end{mapleinput}
%	\begin{maplelatex} ... \end{maplelatex}
%
% and for details about macros such as
%
%	\mapleinline <status> <type> <verbatim code> <latex code>
%	\maplemultiline{ ... }
%
% which are used to control style and to embed raw Maple data.
% 
% USAGE:
%
%	To use this package, add the line  
%
%	\usepackage{maple2e} to 
%
%	your document preamble.  If you are using a specific plot
%	driver such as dvipsone, then add its name as an option as
%	in:
%
%	\usepackage[dvipsone]{maple2e}
%
%	The default option value is "dvips".
%
%	If you wish to preview your document, ignoring plots, use
%	the "noplots" option.
%
%	The only options available are precisely those needed to
%	control plotting.  Plots are handled by the standard LaTeX2e
%	graphics package and for LaTeX are restricted to postscript.
%	 
% NOTES:
%
%	It is an easy extension of this code to other plot file formats.
%	All that is needed is a new definition of \mapleplot
%	to invoke the graphics code of your choice.
%
%	To adjust the spacing around the Maple environemnts, edit
% 	change the entries in the file mapleenv.def
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% Package Options
%
\newif\ifnoplots\noplotsfalse
\DeclareOption{noplots}{
    % \PassOptionsToPackage{dvips}{epsfig}
    \noplotstrue
}
\DeclareOption{dvips}{
    % \PassOptionsToPackage{dvips}{epsfig}
    \edef\Driver{dvips}
    \AtEndOfPackage{
      \typeout{ ...configuring graphics for dvips driver}
      \usepackage[dvips]{epsfig}
      \let\mapleplot\epsfigmapleplot
      \let\imapleplot\mapleplot
    }
}
\DeclareOption{dvi2ps}{
    \edef\Driver{dvi2ps}
    \AtEndOfPackage{
      \typeout{ ...configuring graphics for dvips driver}
      \usepackage[dvi2ps]{epsfig}
      \let\mapleplot\epsfigmapleplot
      \let\imapleplot\mapleplot
    }
}
\DeclareOption{dvilaser}{
    \edef\Driver{dvilaser}
    \AtEndOfPackage{
      \typeout{ ...configuring graphics for dvilaser driver}
      \usepackage[dvilaser]{epsfig}
      \let\mapleplot\epsfigmapleplot
      \let\imapleplot\mapleplot
    }
}
\DeclareOption{dvipsone}{
    \edef\Driver{dvipsone}
    \AtEndOfPackage{
      \typeout{ ...configuring graphics for dvipsone driver}
      \usepackage[dvipsone]{epsfig}
      %%% \let\mapleplot\mapleplotname %%%
      \let\mapleplot\epsfigmapleplot
      \let\imapleplot\mapleplot
    }
}
\DeclareOption{dvitops}{
    \edef\Driver{dvitops}
    \AtEndOfPackage{
      \typeout{ ...configuring graphics for dvitops driver}
      \usepackage[dvitops]{epsfig}
      \let\mapleplot\epsfigmapleplot
      \let\imapleplot\mapleplot
    }
}
\DeclareOption{dviwindo}{
    \edef\Driver{dviwindo}
    \AtEndOfPackage{
      \typeout{ ...configuring graphics for dviwindo driver}
      \usepackage[dviwindo]{epsfig}
      \let\mapleplot\epsfigmapleplot
      \let\imapleplot\mapleplot
    }
}
\DeclareOption{emtex}{
    \edef\Driver{emtex}
    \AtEndOfPackage{
      \typeout{ ...configuring graphics for emtex driver}
      \usepackage[emtex]{epsfig}
      \let\mapleplot\epsfigmapleplot
      \let\imapleplot\mapleplot
    }
}
\DeclareOption{pubps}{
    \edef\Driver{pubps}
    \AtEndOfPackage{
      \typeout{ ...configuring graphics for pubps driver}
      \usepackage[pubps]{epsfig}
      \let\mapleplot\epsfigmapleplot
      \let\imapleplot\mapleplot
    }
}
\DeclareOption{textures}{
    \edef\Driver{textures}
    \AtEndOfPackage{
      \typeout{ ...configuring graphics for textures driver}
      \usepackage[textures]{epsfig}
      \let\mapleplot\epsfigmapleplot
      \let\imapleplot\mapleplot
    }
}
\DeclareOption{xdvi}{
    \edef\Driver{xdvi}
    \AtEndOfPackage{
      \typeout{ ...configuring graphics for xdvi driver}
      \usepackage[xdvi]{epsfig}
      \let\mapleplot\epsfigmapleplot
      \let\imapleplot\mapleplot
    }
}
\DeclareOption{dvitps}{
    \edef\Driver{dvitps}
    \AtEndOfPackage{
      \typeout{ ...configuring graphics for dvitps driver}
      \usepackage[dvitps]{epsfig}
      \let\mapleplot\epsfigmapleplot
      \let\imapleplot\mapleplot
    }
}
\DeclareOption{dviwin}{
    \edef\Driver{dviwin}
    \AtEndOfPackage{
      \typeout{ ...configuring graphics for dviwin driver}
      \usepackage[dviwin]{epsfig}
      \let\mapleplot\epsfigmapleplot
      \let\imapleplot\mapleplot
    }
}
\DeclareOption{oztex}{
    \edef\Driver{oztex}
    \AtEndOfPackage{
      \typeout{ ...Configuring graphics for OzTex, rotation not supported}
      \usepackage[oztex]{epsfig}
      \let\mapleplot\oztexmapleplot
      \let\imapleplot\mapleplot
    }%
}
\DeclareOption{SWP}{
    \edef\Driver{SWP}
    \AtEndOfPackage{
      \typeout{ ...Configuring graphics for Scientific Work Place}
      \let\mapleplot\swpmapleplot
      \let\imapleplot\mapleplot
    }
}
% \ExecuteOptions{dvips}  % default's to dvips driver
\ProcessOptions*
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Utilities and Environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Miscelaneous utilities used to define the main Maple environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\typeout{Defining Maple Utility Macros}
%
% Utilities for changing character codes
%
\def\MakeTab#1{\catcode `#1 = 4 }      		% &
\def\MakeParameter#1{\catcode `#1 = 6 }		% #
\def\MakeSuperScript#1{\catcode `#1 = 7 }	% ^
\def\MakeSubScript#1{\catcode `#1 = 8 }		% _
\def\MakeLetter#1{\catcode `#1 = 11 }
\def\MakeOther#1{\catcode`#1 = 12 }
\def\MakeActive#1{\catcode `#1 = \active\relax }
\def\MakeTabActive{\MakeActive{\^^I}}
\def\MakeEolActive{\MakeActive{\^^M}}
%
\@ifundefined{dospecials}{%
\gdef\dospecials{\do\ \do\\\do\{\do\}\do\$\do\&\do\#\do\^\do\_\do\%\do\~}%
}{\relax}%
\@ifundefined{postdospecials}{%
\gdef\postdospecials{%
\catcode`\\\z@%
\catcode`\{\@ne%
\catcode`\}\tw@%
\catcode`\ 10%
\catcode`\&11}%
}{\relax}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% In a Maple tty environment every line is treated as a paragraph.
% The behavior at the end of every Maple paragraph (line) is given
% by, thereby inhibiting page breaks in such environments.
\def\@MaplePar{\nopagebreak[3]\par\@@par}%
% \def\@MaplePar{\nopagebreak[3]\EveryParZ\@@par}%
%
\newif\if@IgnoreNewLine
\@IgnoreNewLinetrue
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Characters requiring special treatment
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-- Spaces
\def\MapleSpace{\ }
\def\@ObeySpaces{\MakeActive{\ }\@@ObeySpaces\relax}
{\MakeActive{\ }\gdef\@@ObeySpaces{\edef {\MapleSpace}}}

%-- BackSlashes

{\catcode`| = 0 |catcode`\\ = 12 |gdef|BackSlash{\}}

%-- Tabs

\newdimen\@MapleTabSize
\def\@ObeyTabs{\MakeTabActive\@@ObeyTabs\relax}
{\MakeTabActive\gdef\@@ObeyTabs{\def^^I{\@MapleTab}}}
\def\@MapleTab{%
  \leavevmode   % ensure that we are in horizontal mode
  \egroup      % Terminate box register 0
  \dimen0=\wd0 % store its length and round up to next stop
  \divide\dimen0 by \@MapleTabSize
  \advance\dimen0 by 1sp
  \multiply \dimen0 by \@MapleTabSize
  \wd0 = \dimen0
  \box0
  \setbox0 = \hbox\bgroup
}

%-- End of Line Character

\def\@ObeyEol{\MakeEolActive\@@ObeyEol\relax}%
{\MakeEolActive\gdef\@@ObeyEol{\let^^M=\@MapleEol}}
\def\@MapleEol{%
  \if@IgnoreNewLine
  \else
    \leavevmode%
    \egroup%
    \box 0%
    \@MaplePar%
  \fi
  \@IgnoreNewLinefalse
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Definitions of Utilities for the Main Maple Environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% These Macros are the common elements of the verbatim like environents.
% The spacing above and below the environment should is done in the 
% environment preamble instead of here to enable this to be used in a 
% variety of such environments.

% \newtoks\MapleIOType \MapleIOType = {a}
\edef\@MapleQuiet{q}      % indicates a silent command or result
\edef\@MapleVerbose{a}    % The standard behavior in which
                          % results are generated and displayed.
\edef\@MapleNoPrompt{np}  % specify no prompts in environment
\edef\@MaplePrompt{p}     % specify prompts for this environment
\edef\@MapleNoInput{ni}   % No input appears in output stream.
\edef\@MapleNoOutput{no}  % No output appears in outputstream.

% The next macro is used by the verbatim like environments to
% reset character codes, and change the treatment of new lines, etc.
% Actions  can be made conditional on the value of \@MapleIOType which
% is always set to 'a' , or to 'q' as in the value of the 
% optional parameter used in \begin{mapleinput}[q]

\newtoks\MapleListCorrection  \MapleListCorrection={}
\def\@SetupMapleTty#1{%
\par\@endpefalse   %% to clear the \@endpetrue done in \mapleinput
\begingroup  %% this is the real start of the special environment. 
  %%%  Compute and set tab positions
  \setbox 0 = \hbox{\@MapleFont X}
  \@MapleTabSize = \wd0
  \multiply\@MapleTabSize by \MapleTab
  \setbox0 = \hbox{\relax}  % Clearing \box 0
  %%% paragraph dimensions and line spacing
  \rightskip = 0pt 
  \parindent = 0pt
  \parskip = 0pt 
  \ifnum\@listdepth>0%
        \MapleListCorrection={\hskip-\@totalleftmargin\relax }
        \LeftMapleSkip= 0em 
  \else
        \MapleListCorrection={\hskip 0ex\relax }
  \fi
  \setlength{\leftskip}{\LeftMapleSkip}
  \addtolength{\leftskip}{\@totalleftmargin}
  \parfillskip = 0pt plus 1fil
  %
  %%%  The next two parameters may have been changed 
  %%%  by a \raggedright so they are reset here.
  \spaceskip = 0pt   \xspaceskip = 0pt
  %
  %%%  Set this flag to 0 if the \begin{...} is to appear on a
  %%%  separate line of the source file.
  \ifnum #1 = 0 \@IgnoreNewLinetrue\else\@IgnoreNewLinefalse\fi%
  %
  %%% Describe how to handle every paragraph (recall paragraph == line )
  %% \@MapleFont%
  \everypar = {\EveryParZ}%
  \def\EveryParZ{%
    \ifMaplePrompt
    \the\MapleListCorrection
    \the\MaplePromptString
    \MaplePromptString = \MaplePromptSecondary
    \MapleListCorrection = {\hskip 0pt\relax}
    \fi
    \setbox0 = \hbox \bgroup
  }%
%
%%%  Choose the type size and font -  The order of these commands
%%%  may be important.
\@MapleFont%
\lineskiplimit=0\normalbaselineskip%
\baselineskip=0.85\normalbaselineskip%
\@noligs%
\let\do\@makeother\dospecials%
\catcode ``=\active%
\frenchspacing%
\@ObeySpaces% 
\@ObeyTabs%
\@ObeyEol%
}

% Exit the special tty environments
\def\@EndMapleTty{%
\endgroup%% matches the \begingroup inside of @SetupMapleTty
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% The following Macros start the various Verbatim like environments
% for special Maple regions.  These calls set up the 
% scanning for the environment terminator.
%
% A conditional parameter as in \begin{...}[q] etc. denotes a
% special class of Maple Regions.

\begingroup
  \catcode`| = 0  % becomes the escape character
  \catcode`( = 1  % becomes a begin group
  \catcode`) = 2  % becomes an end group
  \catcode`@ = 11 % becomes a regular character (for macro names)
  \catcode`\{ = 12 % becomes an other character
  \catcode`\} = 12 % becomes a other character
  \catcode`\\ = 12 % becomes a other character
%
%  type a   standard (verbose) usage
%  type q   quiet command
%  type np  no prompt  (imapleinput only at this time...)
%  type ni  no input  
%  type no  no output  
%
% -- Maple Inert Input  
|gdef|@BeginIMapleInput#1\end{imapleinput}(%
|MaplePrompttrue%
#1%
|end(imapleinput))%
%
% -- Inert TTY Output
|gdef|@BeginIMapleTtyout#1\end{imaplettyout}(%
|vskip|AboveMapleSkip%  extra vspace is needed here
|MaplePromptfalse
#1%
|end(imaplettyout))%
%
% -- Fixed Width
|gdef|@BeginMapleFixedWidth#1\end{MapleFixedWidth}(%
|vskip|AboveMapleSkip%  extra vspace is needed here
|MaplePromptfalse
#1%
|end(MapleFixedWidth))%
% -- TTY Input 
|gdef|@BeginMapleInput[#1]#2\end{mapleinput}(%
|edef|@MapleIOType(#1)%
|gdef|MapleIOType(#1)%
|ifx|@MapleIOType|@MapleNoPrompt|MaplePromptfalse|fi%
|ifx|@MapleIOType|@MapleNoInput|edef|@MapleIOType(q)|fi%
|ifx|@MapleIOType|@MapleQuiet%
|typeout(.............Quiet Maple Command #1)%
|removelastskip%
|else%
%|typeout(.............Verbose Maple Command)%
#2%
|fi%
|end(mapleinput))%
%
% -- TTY Output
|gdef|@BeginMapleTtyout[#1]#2\end{maplettyout}(%
%%|typeout(TTYout Environment of type #1)%
|edef|@MapleIOType(#1)%
|gdef|MapleIOType(#1)%
|ifx|@MapleIOType|@MaplePrompt|MaplePromptfalse|fi%
|ifx|@MapleIOType|@MapleNoOutput|edef|@MapleIOType(q)|fi%
|ifx|@MapleIOType|@MapleQuiet%
|typeout(.............Quiet Maple Tty Out)%
|else%
#2%
|fi%
|end(maplettyout))%
%
% -- Suppressed Latex Output
|gdef|@GobbleMapleLatex#1\end{maplelatex}(%
|end(maplelatex))%
|endgroup
%
\@ifundefined{]}{\gdef\[{$}}{\relax}
\@ifundefined{[}{\gdef\]{$}}{\relax}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Standard Maple Environments
%
% Environments for Export to LaTeX
%
% This package defines the environments used by Maple's
% "Export to Latex" facility.  In addition, each of the environments 
% accepts an optional parameter.  For example, for example,
% Maple Input lines accept any of:
%
%      \begin{mapleinput}...\end{mapleinput},   (default)
%
% The contents of such an environment are in terms of mapleinline.
%
% The "Export to LaTeX" facility of the Maple worksheet does not use any
% of the optional parameters.  They exist to provide the additional
% control needed for reprocessing long LaTeX manuscripts and which is
% carried out by a special "Maple Filter".
% 
% Maple output can occur in several forms.  Maple's "prettyprint" output,
% as well as error messages and warnings, is encapsulated as
%
% 	        \begin{maplettyout}...\end{maplettyout} 
%
% "Export to Latex" generates LaTeX code for the entire worksheet. 
%  The displayed mathematics output is controlled to fit a
%  user specified line width and appears inside the environment
%
% 	\begin{maplelatex}...\end{maplelatex}
%
% Maple generated plots are exported as postscript files.
% The resulting files are included in the LaTeX document 
% by using the macro call
%
%  	\mapleplot{filename}
%
% On processing by LaTeX, the postscript code from the 
% indicated file is read into "dvi" file and a display is 
% generated at that point in the document.  The plot dimensions 
% are specified as \MaplePlotHeight and \MaplePlotWidth.
%
% The actual embedding is accomplished using the LaTeX2e graphics 
% package.  This style file has been tested with the following dvi to 
% PostScript conversion programs:
%
%     dvips 
%     dvipsone
%
% ----------------------------------------------
% Environments that ignored by the Maple Filter
% ----------------------------------------------
% The Maple Filter is a special version of Maple that can read
% and update latex files which have been developed using these
% macros.  There is a need, in such tex files, to display information
% in the same manner as the preceding manner and yet guarantee that
% the information is not changed by the Maple Filter.
% The macros are identical to those describe above, but with each 
% name preceded by an "i".
%
%   \begin{imapleinput}...\end{imapleinput}  like mapleinput
%   \begin{mapleinput}[p]...\end{imapleinput} as above, default case
%   \begin{imaplelatex}...\end{imaplelatex} like maplelatex
%   \imapleplot{filename}   like mapleplot
%   \imaplesepline	  like \maplesepline, but ignored by the filter.
%
% ----------------------------------------------
% Implementation Details
% ----------------------------------------------
% The mapleinput, and maplettyout environments are similar to 
% \begin{verbatim}...\end{verbatim} but with several 
% important differences.
%
% - The spacing relative to the surrounding environment is different.
%
% - Page breaks are encouraged before commands, or after results,
%   and discouraged inbetween.
%
% - maplettyout and maplelatex environments are assumed to follow
%   mapleinput regions and so have less space above.  This allows us to
%   reduce the space between adjacent Maple regions without any
%   elaborate mechanism to detect when there have been intervening
%   paragraphs of text.
%
% - the size of the font for text regions is definable.  Use \MapleFont
%   to reset the font.
%
% - the  indentation of the environments can be indented by setting 
%   the value of \LeftMapleSkip  .
%
% - a prompt is automatically generated at the start of each line in
%   the case of the input environments.
%
% Much of the spacing and sizing information is parameterized.
% The following Macros control most of the spacing for the 
% Maple environments.  They are all resettable in the preamble of 
% your document. 
% 
% \AboveMapleSkip	- space above an environment
% \BelowMapleSkip	- space below an environment
% \AboveMaplePlot	- space above a Maple Plot 
% \BelowMaplePlot	- space below a Maple Plot
% \MaplePlotHeight	- vertical space reserved for a plot
% \MaplePlotWidth	- width reserved for a plot
% \MaplePlotAngle	- angle of rotatation
% \LeftMapleSkip 	- the amount of left indentation
% \MapleFont 		- The Maple font 
% \MapleSize 		- The size of the Maple font in mapleinput and 
%                          maplettyout
% \MapleLatexSize	- The size of the Maple fonts in maplelatex
% \MapleFirstLine	- controls ingoring first line feed
% \MaplePrompttrue 	- controls insertion of prompt char
% \MaplePromptString	- defines the prompt string
% \MaplePromptSecondary	- defines the secondary prompt string
% \MapleSkip		- amount of glue before and after
%			displayed text
% \MapleTab		- number of spaces per tab (8)
%
% Spacing, dimensions, etc.  
%
% These are all defined and given default values in the file
% mapleenv.def Most may be changed in your document preamble.
%
\input{mapleenv.def}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Define those Maple environments that are to be ignored by
% the Maple Filter.  
% 
% \begin{imapleinput} ...\end{imapleinput}
% \begin{imaplettyout} ...\end{imaplettyout}
% \begin{imaplelatex} ...\end{imaplelatex}
% \imaplesepline
% \imapleplot
%
% These environments are ignored by the Maple Filter.
%
% -- imapleinput
%
\def\imapleinput{
\removelastskip%
\MaplePrompttrue% prompt is required in this environment.
\if@minipage\removelastskip\vskip-1.3ex%
\else\vskip\AboveMapleSkip\fi%
\@SetupMapleTty{0}% The 0 indicates ignore first new line
\@BeginIMapleInput% 
}
%
\def\endimapleinput{%
  \@EndMapleTty%
  \removelastskip%
  \edef\@MapleIOType{\MapleIOType}
  \ifx\@MapleIOType\@MapleQuiet%
    \typeout{ .............Quiet Maple Command finished}
  \else
    \vskip\BelowMapleSkip% not usually followed by output...
  \fi%
  \@endpetrue
  \ignorespaces
}
%
% -- imaplettyout
%
\def\imaplettyout{
  \removelastskip%
  \nopagebreak[3]% 
  \MaplePromptfalse	  % No prompt is required in this environment.
  \@SetupMapleTty{1}   % The 1 indicates "respect first new line"
  \@BeginIMapleTtyout  % np indicates omit prompt
}
%
\def\endimaplettyout{%
  \@EndMapleTty%
  \removelastskip
  \vskip\BelowMapleSkip%
  \pagebreak[3]%
  \@endpetrue
  \ignorespaces
}%
%
% -- imaplelatex
%
%  an inert maple latex environment  (ignored by the filter)
%
\newenvironment{imaplelatex}%
{\vskip.5\AboveMapleSkip\vskip\z@\begin{maplelatex}}{\end{maplelatex}}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define active mapleinput environments.
% 
% \begin{mapleinput} ...\end{mapleinput}
% \begin{maplettyout} ...\end{maplettyout}
% \begin{maplelatex} ...\end{maplelatex}
% 
% These parameterized environments are intended for reprocessing 
% by the Maple Filter.
%
% The [a] case is used by default.  
% The [q] is the quiet (suppressed)  mode.
% The [ni] (no input) behaves the same as [q]
% The [no] behaves the same as [a]
%
% Page breaks are inhibited immediately following the input
% environment.  This assumes that no extra space is 
% required below the region as it is followed by some
% form of Maple output region.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% -- mapleinput
%
\newlength\newleftskip%
\newbox\mapleinputbox%
\newenvironment{mapleinput}{%
%\def\@gobblefirst##1{\relax\egroup\par}
%\def\@gobblesecond##1##2{##1\egroup\par}
\def\@gobblesemicolons##1{##1}
\advance\hsize by -\LeftMapleSkip%
\global\setbox\mapleinputbox=\vbox\bgroup%
\everypar{\the\MaplePromptString\MaplePromptString=\MaplePromptSecondary\ }
\leftskip=\z@%
\parindent=\z@%
\parfillskip=0pt plus 1fil
\lineskiplimit=0\normalbaselineskip
\baselineskip=.85\normalbaselineskip
}{
\egroup% end of vbox
\par\removelastskip
\vskip\AboveMapleSkip%
\newleftskip=\leftskip%
\advance\newleftskip by \LeftMapleSkip%
\advance\newleftskip by \@totalleftmargin% needed for lists
\hbox{\hskip\newleftskip\box\mapleinputbox}
\vskip\BelowMapleSkip}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% -- maplettyout
%
\def\maplettyout{
  \removelastskip%
  \vskip 0pt plus 0pt minus 3pt%  
  \nopagebreak[3]% 
  \MaplePromptfalse	  % No prompt is required in this environment.
  \@SetupMapleTty{1}   % The 1 indicates "respect first new line"
  \@ifnextchar [{\@BeginMapleTtyout}{\@BeginMapleTtyout[a]}%
}
% 
\def\endmaplettyout{%
  \@EndMapleTty%
  \edef\@MapleIOType{\MapleIOType}
  \ifx\@MapleIOType\@MapleQuiet%
     \typeout{ .............Quiet Maple TTY finished}
  \else
    \vskip\BelowMapleSkip%
    \pagebreak[3]%
    \@endpetrue
    \ignorespaces
  \fi
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% -- maplelatex 
%
% This is essentially a wrapper around a display math environment
% It gobbles its content if the [q] or [no] options are in
% effect.
%
\newbox\maplebox
\def\maplelatex{\@ifnextchar [{\@maplelatex}{\@maplelatex[a]}}
%
\def\@maplelatex[#1]{%
\edef\@MapleIOType{#1}%
\gdef\MapleIOType{#1}%% for \ifx test%
\ifx\@MapleIOType\@MapleNoOutput%
\typeout{ .............Output Option [no]}%
\gdef\MapleIOType{q}%%  handle same as \@MapleQuiet  
\fi%
\global\setbox\maplebox=\vbox\bgroup%
\MakeSuperScript{^}%  Ensure these have normal interpretation
\MakeSubScript{_}%
}%
%
\def\endmaplelatex{\egroup%
\edef\@MapleIOType{\MapleIOType}%
\ifx\@MapleIOType\@MapleQuiet%   End the same as the verbatim's
\par%
%\@endpetrue
\else%
%\ifvmode\removelastskip\fi%
\nopagebreak[3]%
\centerline{%
\vbox{%
\hbox{\vrule height4pt depth0pt width 0pt}%
\unvbox\maplebox}}%
\vskip\BelowMapleSkip%
\everypar{}%
\par%

%\pagebreak[3]%
%\@endpetrue
%\ignorespaces
\fi%
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% -- maplesepline
%
\newcommand{\maplesepline}{\vskip \parskip%
\hrule\@height\MapleSepLineHeight\@width\MapleSepLineWidth%
\vskip \parskip\relax}
%
% -- imaplesepline ( the inert form )
%
\let\imaplesepline\maplesepline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% -- \mapleIndent
%
% - Special Indentation Macro used to format procedures
%
\newdimen\Tab
\Tab=3ex
\def\mapleIndent#1{\hbox{\hskip#1\Tab\relax}}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Special environments for in-line maple commands.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  \begin{maplegroup}				- maple exchange group
%  ...
%  ... and \mexpr{sin(x^2)} ...			- inline maple code
%  ...
%  \mapleinline{Inert}{TwoD}{int(sin(x^2),x);}{%	- for maple filter
%  {mapletex}{$\int{ .... }$}		        - for latex
%  ...
%  ...
%  \mapleresult					- location of inline results
%  \begin{maplelatex}				- actual displayed results
%  ...
%  \end{maplelatex}
%  \end{maplegroup}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% -- \mexpr 
%
% 	\mexpr{int(sin(x^2),x)} --- \mapleexpr{int(sin(x^2),x)}
%
% To make { and } visible in this verbatim environment, use \{ and \}
% Also, to make \ visible, use \\. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\def\mexpr{\setbox\@inlinebox=\hbox\bgroup\ttfamily\dosetup\let\\\BackSlash\@domexpr}
%
\def\mapleexpr{\bgroup\ttfamily\dosetup\let\\\BackSlash\@domexpr}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  \@dosetup	      sets up the character codes, etc. for verbatim
%  \@domexpr          completes the following inline math
%  \@gobblefirst      absorbs the inline math (not displaying it)
%  \@gobblesecond     absorbs the second following argument.
%  \@gobblesemicolons      absorbs semi-colons inside of the 1d mode.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\dosetup{\let\do\@makeother\dospecials\postdospecials}
%
%\def\@domexpr#1{#1\egroup\fbox{\box\@inlinebox}}
\def\@domexpr#1{#1\egroup\box\@inlinebox}
%
\def\@gobblefirst#1{%
\relax\egroup%
% \fbox{\box\@inlinebox}%   %%% DEBUG %%%
\box\@inlinebox%
\setbox\@inlinebox=\hbox{}}
%
\def\@gobblesecond#1#2{%
#1\egroup\ignorespaces%
% \fbox{\box\@inlinebox}% %%% DEBUG %%%
\box\@inlinebox%
\setbox\@inlinebox=\hbox{}}
%
\def\@gobblesemicolons{\MakeActive{;}\@@gobblesemicolons}
%
{\MakeActive{;}\gdef\@@gobblesemicolons{\edef;{\relax}}}

%%% end of mexpr
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% -- \mapleinline
%
%	Essentially a four argument macro used to control the
%	display of inline material generated by Maple.
%
%	\mapleinline %
%	<status> 	% "active", or "inert"
%	<display mode>  % 1d or 2d
%	<verbatim source> % raw maple code as per \mexpr
%	<latex 2-D source> % latex representation
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% \mapleinline{inert}{2d}{int(sin(x^2),x)}{ % used to generate display
% $\int{\sin(x^2),dx}$}	                    % updated by the filter
%
% Could use \@bsphack ... \@esphack for absorbing unwanted space not 
% currently used, but spacing inside this macro definition is 
% very important.
%
\edef\OneD{1d}\edef\TwoD{2d}% # tokens to identify modes
\newif\ifDisplay\Displayfalse
\newbox\@inlinebox\setbox\@inlinebox=\hbox{}%
\@ifundefined{@skiponetoken}{\gdef\@skiponetoken#1{\relax}}{\relax}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 2-D output
% final output macro for mapleinline.
% include spacing above and below to ensure there is
% whitespace around the object when it occurs in
% a spreadsheet cell.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@doTwoD#1{\egroup%
%\@ifnextchar\cr{\@skiponetoken}{\relax}%
\@@doTwoD}%
%
\newdimen\cellwidth%
\def\@@doTwoD#1{%
\ignorespaces%
\setbox\@inlinebox=\hbox{#1}%
\ifMapleTableCell%  		  Used in maplespreadsheet
\cellwidth=\wd\@inlinebox%
\hbox{$\vcenter{\hsize=\cellwidth%
\hbox{\vrule height3pt depth0pt width 0pt}%
\box\@inlinebox%
\hbox{\vrule height0pt depth 3pt width 0pt}%  Actual output
}$}%
\egroup%
\else%				  Used inline ...
%\fbox{\hbox{\unhbox\@inlinebox}}\egroup% Actual output
\box\@inlinebox\egroup%
\fi%
}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 1-D output
% Final output macro for mapleinline for 1-D output.
% The raw tokens must be dumped into the output stream so
% we use unhbox.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@doOneD#1{\MakeOther{\ } #1\egroup\unvbox\@inlinebox\relax\@mgobbleone}
\def\@mgobbleone#1{\relax\egroup}
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\mapleinline#1#2{%
% ignore first argument (inert or active)		
\def\[{$}\def\]{$}%		% needed for math mode.
\edef\DisplayType{#2}%		% 1d or 2d
\ifx\DisplayType\TwoD%
\let\Display\@doTwoD%	% display the 2-D representation
\global\Displaytrue%
\else%
\let\Display\@doOneD%	% display the 1-D representation
\global\Displayfalse%
\fi%
\bgroup%
\global\setbox\@inlinebox=\vbox\bgroup%
\obeylines%
\everypar{\the\MaplePromptString\MaplePromptString=\MaplePromptSecondary\ }
\ttfamily\dosetup\obeyspaces\let\\\BackSlash\Display%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% -- \begin{maplegroup} ... \end{maplegroup}
% -- \mapleresult
%
%	A environment used to group commands and result together into
%	one unit.  Inside, these are separated by \mapleresult.
%	The maple filter automatically deletes the part of a maplegroup
%	which follows \mapleresult and replaces it with new results.
%	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newenvironment{maplegroup}{}{}
\def\maplegroup{\relax}
\def\endmaplegroup{\relax}
\let\mapleresult\relax   

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Various Plot Configurations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\typeout{Defining Maple Plot Environemnts}
% 
% -- noplots  -- No Driver Available ?
%
\def\mapleplotname#1{
	\typeout{ ...using Plot file #1}%
	\vskip.5\MaplePlotHeight
        \centerline{\Large \bfseries Plot:  #1}
        \vskip.5\MaplePlotHeight
}
%
% -- epsfig.sty (used by dvips, etc)
%
\def\epsfigmapleplot#1{
	\parindent=0ex%
	\MaplePlotWidth  = 0.900\textwidth%
	\MaplePlotHeight = 0.651\textwidth%
	\MaplePlotHeight@Fudge=0.90\MaplePlotHeight%
	\MaplePlotWidth@Fudge =0.90\MaplePlotWidth%
	\ifvmode \removelastskip \else \par \parindent=0ex\removelastskip\fi
	%% \par
        \vskip \AboveMaplePlot
	%
	%  Plot sizes must be fudged because Maple .eps plots
	%  generated using Maple's built-in PostScript plot driver
	%  are 6.5 x 9 inches landscape, but included in portrait
	%  mode to a much smaller scale.
	%
	\IfFileExists{#1}{%
		\typeout{ ...including Plot #1 at size
		\the\MaplePlotWidth\space by \the\MaplePlotHeight}%
		\hbox{%
		    \relax
		    {}\hskip \LeftMapleSkip
		    \epsfig{figure=#1,%
			height=\MaplePlotHeight@Fudge,% scale before rotation
			width=\MaplePlotWidth@Fudge,%
			angle=\MaplePlotAngle}%
		}% end of hbox
	}% 
	{%
		\typeout{ ...Missing Plot File  #1}
		\noindent	% So \mapleplot can be used inside of
				% the LaTeX center environment.
		\vbox{\mapleplotname{#1} }%
	}%
	\par\removelastskip
        \vskip\BelowMaplePlot
	% \vskip-2\BelowMaplePlot{\relax}
	%%% \vspace*{-.3\MaplePlotHeight} 
	% \relax\noindent\ignorespaces
}% end of epsfigmapleplot def

%%
%Driver used exclusively by plots in Maple 11. The dimensions of the 
%plot are specified as point sizes in the 2nd and 3rd parameters.
%This driver is virtually the same as epsfigmapleplot, but without the rotation
%and the dimension fudge. 
%%
\def\maplepsplot#1#2#3{
	\parindent=0ex%
	\MaplePlotWidth  = #2%
	\MaplePlotHeight = #3%
	\ifvmode \removelastskip \else \par \parindent=0ex\removelastskip\fi
        \vskip \AboveMaplePlot
	\IfFileExists{#1}{%
		\typeout{ ...including Plot #1 at size
		\the\MaplePlotWidth\space by \the\MaplePlotHeight}%
		\hbox{%
		    \relax
		    {}\hskip \LeftMapleSkip
		    \epsfig{
		    	figure=#1,%
			height=\MaplePlotHeight,
			width=\MaplePlotWidth
		    }%
		}% end of hbox
	}% 
	{%
		\typeout{ ...Missing Plot File  #1}
		\noindent	% So \mapleplot can be used inside of
				% the LaTeX center environment.
		\vbox{\mapleplotname{#1} }%
	}%
	\par\removelastskip
        \vskip\BelowMaplePlot
}% end of maplepsplot def

%
% -- Oztex postscript driver
%
% Rotation is not supported.  so use Maple's commands to rotate.
% This can be done using the Maple command 
%
%	interface(plotoptions=`portrait,height=200,width=300`); 
%
% This is the same as mapleespfig, but with no rotation expected.
%
\def\oztexmapleplot#1{
	\ifvmode \removelastskip \else \par \fi
	\vskip \AboveMaplePlot
	%
	%  Plot sizes must be fudged because Maple .eps plots
	%  generated using Maple's built-in PostScript plot driver
	%  are 7.5 x 10 inches, but include an additional 0.5 inch
	%  white border within the PostScript BoundingBox.
	%
	\MaplePlotHeight@Fudge=1.133333\MaplePlotHeight
	\MaplePlotWidth@Fudge =1.100000\MaplePlotWidth
	\vskip -0.066667\MaplePlotHeight		%Fudge
	\noindent	% So \mapleplot can be used inside of
			% the LaTeX center environment.
	\IfFileExists{#1}{%
		\typeout{ ...including Plot #1 at size
		\the\MaplePlotWidth\space by \the\MaplePlotHeight}%
		\hbox{%
		    \hskip -0.05\MaplePlotWidth		%Fudge
		    \epsfig{figure=#1,%
			height=\MaplePlotWidth@Fudge,% scale before rotation
			width=\MaplePlotHeight@Fudge}%
%%oztex%% 			angle=\MaplePlotAngle}%
		    \hskip -0.05\MaplePlotWidth		%Fudge
		}%
	}% end of first case
	{% second case 
	    %\typeout{ ...Missing Plot File  #1}
	    { %
		\vskip.5\MaplePlotHeight%
		\centerline{\Large \bfseries Plot File = #1}
		\vskip.5\MaplePlotHeight %
		}% end of vbox
	}% end of second case
	\par
	\vskip -0.066667\MaplePlotHeight		%Fudge
	\vskip\BelowMaplePlot
	\vskip -\parskip\noindent\ignorespaces
} % end of oztexmapleplot

%%%%%%%%%%%%%%%%%%%%%%%%%
% Install the Driver.
%%%%%%%%%%%%%%%%%%%%%%%%%
\@ifundefined{Driver}{%
      \ifnoplots
	     \let\mapleplot\mapleplotname
	     \let\imapleplot\mapleplot
      \else
      \IfFileExists{epsfig.sty}{% Default to dvips
             \typeout{ ...Defaults to "dvips" Driver }
             \usepackage[dvips]{epsfig}
             \let\mapleplot\epsfigmapleplot
             \let\imapleplot\mapleplot
             \edef\Driver{dvips}}{%  no driver 
	     % generate vertical space containing file name
	     \let\mapleplot\mapleplotname
	     \let\imapleplot\mapleplot
	}
      \fi
}{\usepackage[\Driver]{epsfig}}
%
\def\maplesmartplot#1#2{\mapleplotname{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Maple Paragraph Styles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\typeout{Defining Automatic Style Generation Macros}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%--  Maple Worksheet Default Paragraph and Character Styles definitions
%
%   Unnamed Character styles are set up as {\textbf ... } while
%   named character styles are set up as macro calls of the form
%
%             \QTR{Style Name}{ ... data ... }
%
%   Paragraph styles are tagged by environments as in
%
%   \begin{flushleft} ... \end{flushleft}
%
%   This tagging also occurs for the user defined styles.
%
%   A list of style names actually used in a particular worksheet is
%   specified at the top of a Maple worksheet by macros of the form
%
%   \DefineCharStyle{... style name ...}
%   \DefineParaStyle{... style name ...}
%
%   If a macro by that name is already defined, then that definition
%   is used. Otherwise, a new macro is defined and set to the
%   document default style.
%
%   All style definitions, user defined, or system defined in this
%   style file, can be overridden in the document preamble simply
%   by providing a definition prior to The \Define...Style{...}
%   call.
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%--------------------------------------------------------------------
% - Routine for Automatically defining Undefined Character Styles
%--------------------------------------------------------------------
\newif\if@def\@deffalse
\def\DefineCharStyle#1{
  \@ifundefined{#1}{\@deftrue}{\@deffalse}
  \if@def
    \typeout{Defining a new character style: #1}
    \expandafter\def\csname #1\endcsname##1{\relax {##1}}
  \fi}
%
%--------------------------------------------------------------------
% - Routine for Handling Undefined Paragraph Styles  
%
% These are handled as environments.  Blank spaces are allowed in 
% the environment names.
%--------------------------------------------------------------------
\def\DefineParaStyle#1{
\@ifundefined{#1}{\@deftrue}{\@deffalse}
\if@def
  \typeout{Defining new paragraph style: #1}
  \expandafter\newcommand \csname #1\endcsname[0]{\relax}%
  \expandafter\long\expandafter\def\csname end#1\endcsname{\relax}
\fi
}

%--------------------------------------------------------------------
% - Routine for Handling Undefined Character Styles
%
% This macro allows for macro names having spaces in them.
% Usage:
%
%     \QTR{macro name}{argument 1}
%
%--------------------------------------------------------------------
\@ifundefined{QTR}{%	
  \gdef\QTR#1#2{{\csname#1\endcsname{#2}}}}{\relax} % 
\@ifundefined{TEXTsymbol}{%
  \gdef\TEXTsymbol#1{\mbox{$#1$}}}{\relax}%

%--------------------------------------------------------------------
% - The Known (Pre-defined!) Maple Paragraph Styles
%---------------------------------------------------------------------
% \newenvironment{maplegroup}{}{}
\newenvironment{Maple Author}{\begin{center}\large\itshape\mdseries}{\end{center}}
\newenvironment{Maple subtitle}{\begin{center}\normalsize\upshape\mdseries}{\end{center}}
\newenvironment{Maple Bullet Item}{%
\renewcommand{\labelitemi}{$\bullet$}
\begin{itemize}\item\null}{\end{itemize}}
\newenvironment{Maple Dash Item}{%
\begin{itemize}\item\null}{\end{itemize}}
\newenvironment{Maple Diagnostic}{\bfseries}{}
\newenvironment{Maple Error}{\bfseries}{}
%
\newenvironment{Maple Heading 1}[2][\section]
{#1{\Large\bfseries\upshape {#2}}}
{}
\newenvironment{Maple Heading 2}[2][\subsection]
{#1{\large\bfseries\upshape {#2}}}
{}
\newenvironment{Maple Heading 3}[2][\subsubsection]
{#1{\normalsize\bfseries\upshape {#2}}}
{}
\newenvironment{Maple Heading 4}[2][\subsubsection]
{#1{\normalsize\bfseries\itshape {#2}}}
{}
%
\newenvironment{Maple Normal}{\normalsize\rmfamily\mdseries}{}
\newenvironment{Maple Text Output}{\normalsize\ttfamily\mdseries}{}
\newenvironment{Maple Title}{\begin{center}\rmfamily\LARGE\upshape\ignorespaces}%
{\end{center}}
\newenvironment{Maple Warning}{\ttfamily}{}
%--------------------------------------------------------------------
% -- Fixed Width Environment is like a verbatim Version
%--------------------------------------------------------------------
%
\newbox\maplettybox%
\setbox\maplettybox=\hbox{}
%
\expandafter\def\csname MapleFixedWidth\endcsname{
  \removelastskip%
  \nopagebreak[3]% 
  \MaplePromptfalse	  % No prompt is required in this environment.
  \@SetupMapleTty{1}   % The 1 indicates "respect first new line"
  \@BeginMapleFixedWidth  % np indicates omit prompt
}
%
\expandafter\def\csname endMapleFixedWidth\endcsname{%
  \@EndMapleTty%
  \removelastskip
  \vskip\BelowMapleSkip%
  \pagebreak[3]%
  \@endpetrue
  \ignorespaces
}%
%
%------------------------------------------------------------------------------
% -- Regular Known Character styles
%
%        If spaces occur in name then define using \expandafter
%        as seen below, and invoke as QTR{name}{options}
%	 Otherwise, define and use as normal (i.e., using \def)
%
%------------------------------------------------------------------------------
\expandafter\def\csname Maple 2D Comment\endcsname#1{{\rmfamily\upshape #1}}
\expandafter\def\csname Maple 2D Input\endcsname#1{{\rmfamily\upshape #1}}
\expandafter\def\csname Maple 2D Math\endcsname#1{{\rmfamily\upshape #1}}
\expandafter\def\csname Maple 2D Output\endcsname#1{{\rmfamily\upshape #1}}
\expandafter\def\csname Maple Help Heading\endcsname#1{{\large\bfseries\sffamily\upshape #1}}
\expandafter\def\csname Maple Help Normal\endcsname#1{{\rmfamily\itshape #1}}
\expandafter\def\csname Maple 2D Comment\endcsname#1{{\rmfamily\itshape #1}}
\expandafter\def\csname Maple Maple Input\endcsname#1{{\ttfamily\upshape #1}}
\expandafter\def\csname Maple Output Labels\endcsname#1{{\ttfamily\upshape #1}}
\expandafter\def\csname Maple Plot Title\endcsname#1{{\large\sffamily\upshape #1}}
\expandafter\def\csname Maple Plot Text\endcsname#1{{\sffamily\upshape #1}}
\expandafter\def\csname Maple Popup\endcsname#1{{\bfseries\sffamily\upshape #1}}
\expandafter\def\csname Maple Hyperlink\endcsname#1{{\bfseries\rmfamily\itshape #1}}
%--------------------------------------------------------------------
% Hyperlink support (printing characteristics only)
%--------------------------------------------------------------------
\def\labelLink#1#2{\Hyperlink{#2}}
\def\docLink#1#2{\Hyperlink{#2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Maple Table Support
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\typeout{Defining Maple Spreadsheet Environments}
\typeout{Maple Spreadsheet and Table Support}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Maple Spreadsheets and Tables Package
%%%
%%%  Maple displays its spreadsheets as a tabular arrays of cells.
%%%
%%% This is essentially a tabular environment
%%% with some pre and post processing. 
%%% The format is:
%%% \begin{maplespreadsheet}[spreadsheet01.tab]{|c|c|}
%%% \hline
%%% entry 1 &
%%% entry 2 &
%%% \mapleinline{inert}{2d}{1;}{xx} \\
%%% \hline
%%% entry 2,21 &
%%% entry 2,3  &
%%% \mapleinline{{1;} \\
%%% \hline
%%%\end{maplespreadsheet}
%%%
%%%  The cells are in typeset in text mode. The mathematics is
%%%  usually provided in \mapleinline in order to provide both the
%%%  Maple and the LaTeX encoding of the expression.
%%%
%%%  Maple's \multiline macro is used in the latex portion
%%%  of the \mapleinline macro in order to effect line wrapping.
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\ifMapleTableCell%  % used to change vertical offset of a
			  % mapleinline inside table
\newdimen\multilinesep%
\multilinesep=1ex%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% maplespreadsheet - tabular environment whose entries are encoded
%%%	using mapleinline.
%%%
%%%	\begin{maplespreadsheet}[filename]{format}
%%%	...
%%%	\end{maplespreadsheet}
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\maplespreadsheet{%
\@ifnextchar [{\@maplespreadsheet}{\@maplespreadsheet[]}
}
\def\@maplespreadsheet[#1]#2{%
\par\MapleTableCelltrue\begin{center}\begin{tabular}{#2}}%
\def\endmaplespreadsheet{%
\end{tabular}%
\end{center}%
\MapleTableCellfalse%
}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% maplemultiline - Used for stacking lines of maple input and output
%%%
%%% An implementation of mapleinline based on vbox and hbox.
%%% The tokens are parsed and dropped into hboxes which are in turn
%%% collected into a vbox.
%%%
%%% Each line of the multiline is followed by some extra space
%%% No extra space is required at the top as the multiline is
%%% used inside of \mapleinline, which provide's its own space
%%%
%%% \maplemultiline{x^2 + y^2\\(x - y)^{100}\\}
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Tokens and utilities used by \maplemultiinline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newbox\@linebuffer\setbox\@linebuffer=\vbox{\relax}
\newbox\@currentline\setbox\@currentline=\hbox{\relax}
\newdimen\@linebufferwidth  %%% DEBUG %%%
\newtoks\EndMultiLine%
\@ifundefined{@skiponetoken}{\gdef\@skiponetoken#1{\relax}}{\relax}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \maplemultiline -
%%% for use primarily inside of table cells.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\maplemultiline#1{%
{\def\\{\relax}%
\processcell#1\noexpand\\\EndMultiLine%
}%
%%% \@linebufferwidth=\wd\@linebuffer%%% DEBUG %%%
%\fbox{\@dumplinebuffer}%         %%% DEBUG %%%
\@dumplinebuffer%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \processcell -
%%% start processing the contents of the cell
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\processcell{\futurelet\@nexttoken\processline}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \processline
%%% - invokes \processfullline unless at the
%%% end of the cell. (skips over \cr's to
%%% avoid spacing problems)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\processline{%
\ifx\@nexttoken\EndMultiLine%
\let\next\@skiponetoken%  % at end of cell.
\else%
\let\next\processfullline%% grab next line 
\fi%
% \cr's cause spacing problems.
\ifx\@nexttoken\cr\@skiponetoken\let\next\processline\fi%
\next%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \processfullline -
%%% - Adds currentline (as identified by \\)
%%% to the vbox \@linebuffer
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\processfullline #1\\{%
\global\setbox\@currentline=\hbox{$#1$}
\@extendlinebuffer{\@currentline}%
\processcell}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \@extendlinebuffer - a stack of lines
%%% add currentline to end of \@linebuffer
%%%
%%% #1 is assumed to be a box. (hbox) and
%%% is reset at the end.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@extendlinebuffer#1{%
\ifvoid#1\else% 	% skip over blank lines
\ifvoid\@linebuffer%	% first line ?
\global\setbox\@linebuffer=\vtop{\copy#1}%
\else%			% add new lines
\global\setbox\@linebuffer=\vtop{%
\unvcopy\@linebuffer%
\copy#1%
\vskip\multilinesep%
}%
\fi%
\fi%
\global\setbox#1=\hbox{}% reset currentline
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \@dumplinebuffer -
%%% place @linebuffer on the output stream as
%%% a vbox.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@dumplinebuffer{%
\setbox\@linebuffer=\vtop{%
\hbox{\vrule height3pt depth0pt width 0pt}%
\unvbox\@linebuffer%
\unskip}%  
\box\@linebuffer%  A verticle box ...
\global\setbox\@linebuffer=\vbox{}%
\relax}

\newcommand{\Mapleoversetsp}[2]%
  {\mathop{\kern\z@#2}\limits^{\!\!\!#1}}
\newcommand{\Mapleundersetsp}[2]%
  {\mathop{\kern\z@#2}\limits_{\!\!\!#1}}

\newcommand{\Mapleoverset}[2]%
  {\mathop{\kern\z@#2}\limits^{#1}}
\newcommand{\Mapleunderset}[2]%
  {\mathop{\kern\z@#2}\limits_{#1}}

\endinput 
%%%% The End %%%%%
%%% </PRE>
